The Dependence of Machine Learning on Electronic Medical Record Quality

There is growing interest in applying machine learning methods to Electronic Medical Records (EMR). Across different institutions, however, EMR quality can vary widely. This work investigated the impact of this disparity on the performance of three advanced machine learning algorithms: logistic regression, multilayer perceptron, and recurrent neural network. The EMR disparity was emulated using different permutations of the EMR collected at Children's Hospital Los Angeles (CHLA) Pediatric Intensive Care Unit (PICU) and Cardiothoracic Intensive Care Unit (CTICU). The algorithms were trained using patients from the PICU to predict in-ICU mortality for patients in a held out set of PICU and CTICU patients. The disparate patient populations between the PICU and CTICU provide an estimate of generalization errors across different ICUs. We quantified and evaluated the generalization of these algorithms on varying EMR size, input types, and fidelity of data.

==> deprecated_5_methods.tex <==
% \section*{Methods}
% The algorithms were trained using the pre-processed EMR described in previous sections. The inputs were the patient-matrices (illustrated in Figure \ref{fig:data_imputation}). The target vector was the patient's in-ICU mortality, repeated for each time-step. We leveraged Keras (with Theano backend), a high-level deep learning python package, to train the models on NVIDIA Titan Xs. Each model and data permutation were trained 5 times. Each iteration was evaluated on the PICU and CTICU test set with the mean performance and standard deviation reported.

% The models were trained using mini-batch size of 128 and optimized using RMSprop \cite{tieleman2012lecture} to minimize the binary cross-entropy of predicting in-ICU mortality. As a data augmentation method, a dropout of  $20\%$ was applied to the input sequences (across time) as a data augmentation parameter. \textbf{This-simulates-what}.

% The RNN model consists of two stacked LSTM layers, each with hidden units of 397 (equal to the number of variables in the input vector), and a dense layer (also known as fully-connected layer). The MLP is composed of two stacked dense layers with hidden units of 256, and a final dense layer for classification. The diagram for each model is shown in Figure \ref{fig:model_architectures}. The weights for each model were initialized using Glorot uniform (also known as Xavier).\cite{glorot2010understanding} The RNN was initialized with a learning rate of $10e^{-5}$ and MLP and LR were initialized with a learning rate of $10e^{-4}$. Learning rates were reduced by 5 if the binary cross-entropy on the validation data did not decrease after 15 epochs (an epoch is defined as a cycle through the training set). After 2 reductions, the model's weights associated with the best validation performance was saved.

% The algorithms were evaluated based on the Area Under the Receiver Operating Curve (AUROC) of their in-ICU mortality prediction after 12 hours of observation. 

